Visualisation of Brain Statistics with R-packages ggseg and ggseg3d

There is an increased emphasis on visualizing neuroimaging results in more intuitive ways. Common statistical tools for dissemination, such as bar charts, lack the spatial dimension that is inherent in neuroimaging data. Here we present two packages for the statistical software R, ggseg and ggseg3d, that integrate this spatial component. The ggseg and ggseg3d packages visualize pre-defined brain segmentations as both 2D polygons and 3D meshes, respectively. Both packages are integrated with other well-established R-packages, allowing great flexibility. In this tutorial, we present the main data and functions in the ggseg and ggseg3d packages for brain atlas visualization. The main highlighted functions are able to display brain segmentation plots in R. Further, the accompanying ggsegExtra-package includes a wider collection of atlases, and is intended for community-based efforts to develop more compatible atlases to ggseg and ggseg3d. Overall, the ggseg-packages facilitate parcellation-based visualizations in R, improve and ease the dissemination of the results, and increase the efficiency of the workflows.

==> references <==
@article{eickhoff_2018,
	title = {Imaging-based parcellations of the human brain},
	volume = {19},
	issn = {1471-0048},
	url = {https://doi.org/10.1038/s41583-018-0071-7},
	doi = {10.1038/s41583-018-0071-7},
	abstract = {A defining aspect of brain organization is its spatial heterogeneity, which gives rise to multiple topographies at different scales. Brain parcellation — defining distinct partitions in the brain, be they areas or networks that comprise multiple discontinuous but closely interacting regions — is thus fundamental for understanding brain organization and function. The past decade has seen an explosion of in vivo MRI-based approaches to identify and parcellate the brain on the basis of a wealth of different features, ranging from local properties of brain tissue to long-range connectivity patterns, in addition to structural and functional markers. Given the high diversity of these various approaches, assessing the convergence and divergence among these ensuing maps is a challenge. Inter-individual variability adds to this challenge but also provides new opportunities when coupled with cross-species and developmental parcellation studies.},
	number = {11},
	journal = {Nature Reviews Neuroscience},
	author = {Eickhoff, Simon B. and Yeo, B. T. Thomas and Genon, Sarah},
	month = nov,
	year = {2018},
	pages = {672--686}
}
@article{Fischl2000,
  author = {Fischl, Bruce and Dale, Anders M.}, 
  title = {{Measuring the thickness of the human cerebral cortex from magnetic resonance images}}, 
  volume = {97}, 
  number = {20}, 
  pages = {11050-11055}, 
  year = {2000}, 
  eprint = {http://www.pnas.org/content/97/20/11050.full.pdf+html}, 
  journal = {Proceedings of the National Academy of Sciences of the United States of America}
}
@article{WALHOVD20051261,
title = "Effects of age on volumes of cortex, white matter and subcortical structures",
journal = "Neurobiology of Aging",
volume = "26",
number = "9",
pages = "1261 - 1270",
year = "2005",
issn = "0197-4580",
doi = "https://doi.org/10.1016/j.neurobiolaging.2005.05.020",
url = "http://www.sciencedirect.com/science/article/pii/S0197458005001673",
author = "Kristine B. Walhovd and Anders M. Fjell and Ivar Reinvang and Arvid Lundervold and Anders M. Dale and Dag E. Eilertsen and Brian T. Quinn and David Salat and Nikos Makris and Bruce Fischl",
keywords = "MRI, Morphometry, Age, Cortex, White matter, Cerebellum, Ventricles, Hippocampus, Amygdala, Thalamus, Accumbens area, Striatum, Pons",
abstract = "The effect of age was investigated in and compared across 16 automatically segmented brain measures: cortical gray matter, cerebral white matter, hippocampus, amygdala, thalamus, the accumbens area, caudate, putamen, pallidum, brainstem, cerebellar cortex, cerebellar white matter, the lateral ventricle, the inferior lateral ventricle, and the 3rd and 4th ventricle. Significant age effects were found for all volumes except pallidum and the 4th ventricle. Heterogeneous age responses were seen in that age relationships for cortex, amygdala, thalamus, the accumbens area, and caudate were linear, while cerebral white matter, hippocampus, brainstem, cerebellar white, and gray matter, as well as volume of the lateral, inferior lateral, and 3rd ventricles showed curvilinear relationships with age. In general, the findings point to global and large effects of age across brain volumes."
}
@article{Pizzagalli,
author = {Pizzagalli, Diego  A. and Holmes, Avram  J. and Dillon, Daniel  G. and Goetz, Elena  L. and Birk, Jeffrey  L. and Bogdan, Ryan and Dougherty, Darin  D. and Iosifescu, Dan  V. and Rauch, Scott  L. and Fava, Maurizio},
title = {Reduced Caudate and Nucleus Accumbens Response to Rewards in Unmedicated Individuals With Major Depressive Disorder},
journal = {American Journal of Psychiatry},
volume = {166},
number = {6},
pages = {702-710},
year = {2009},
doi = {10.1176/appi.ajp.2008.08081201},
note ={PMID: 19411368},
URL = {https://doi.org/10.1176/appi.ajp.2008.08081201},
eprint = {https://doi.org/10.1176/appi.ajp.2008.08081201},
abstract = { Objective: Major depressive disorder is characterized by impaired reward processing, possibly due to dysfunction in the basal ganglia. However, few neuroimaging studies of depression have distinguished between anticipatory and consummatory phases of reward processing. Using functional MRI (fMRI) and a task that dissociates anticipatory and consummatory phases of reward processing, the authors tested the hypothesis that individuals with major depression would show reduced reward-related responses in basal ganglia structures. Method: A monetary incentive delay task was presented to 30 unmedicated individuals with major depressive disorder and 31 healthy comparison subjects during fMRI scanning. Whole-brain analyses focused on neural responses to reward-predicting cues and rewarding outcomes (i.e., monetary gains). Secondary analyses focused on the relationship between anhedonic symptoms and basal ganglia volumes. Results: Relative to comparison subjects, participants with major depression showed significantly weaker responses to gains in the left nucleus accumbens and the caudate bilaterally. Group differences in these regions were specific to rewarding outcomes and did not generalize to neutral or negative outcomes, although relatively reduced responses to monetary penalties in the major depression group emerged in other caudate regions. By contrast, evidence for group differences during reward anticipation was weaker, although participants with major depression showed reduced activation to reward cues in a small sector of the left posterior putamen. In the major depression group, anhedonic symptoms and depression severity were associated with reduced caudate volume bilaterally. Conclusions: These results suggest that basal ganglia dysfunction in major depression may affect the consummatory phase of reward processing. Additionally, morphometric results suggest that anhedonia in major depression is related to caudate volume. }
}

@Article{dale_99,
  AUTHOR = "Dale, Anders and Fischl, Bruce and Sereno, Martin I.",
  TITLE = "Cortical Surface-Based Analysis: I. Segmentation and Surface Reconstruction",
  YEAR = "1999",
  JOURNAL = "NeuroImage",
  VOLUME = "9",
  NUMBER = "2",
  PAGES = "179 - 194",
  ANNOTE = "DOI: 10.1006/nimg.1998.0395"
}
@Article{fischl_99,
      AUTHOR = "Fischl, Bruce and Sereno, Martin I. and Dale, Anders",
      TITLE = "Cortical Surface-Based Analysis: II: Inflation, Flattening, and a Surface-Based Coordinate System",
      YEAR = "1999",
      JOURNAL = "NeuroImage",
      VOLUME = "9",
      NUMBER = "2",
      PAGES = "195 - 207",
      ANNOTE = "DOI: 10.1006/nimg.1998.0396"
}
@article{aseg,
  title = "Whole Brain Segmentation: Automated Labeling of Neuroanatomical Structures in the Human Brain",
  journal = "Neuron",
  volume = "33",
  number = "3",
  pages = "341 - 355",
  year = "2002",
  issn = "0896-6273",
  doi = "https://doi.org/10.1016/S0896-6273(02)00569-X",
  url = "http://www.sciencedirect.com/science/article/pii/S089662730200569X",
  author = "Bruce Fischl and David H. Salat and Evelina Busa and Marilyn Albert and Megan Dieterich and Christian Haselgrove and Andre van der Kouwe and Ron Killiany and David Kennedy and Shuna Klaveness and Albert Montillo and Nikos Makris and Bruce Rosen and Anders M. Dale",
  abstract = "We present a technique for automatically assigning a neuroanatomical label to each voxel in an MRI volume based on probabilistic information automatically estimated from a manually labeled training set. In contrast to existing segmentation procedures that only label a small number of tissue classes, the current method assigns one of 37 labels to each voxel, including left and right caudate, putamen, pallidum, thalamus, lateral ventricles, hippocampus, and amygdala. The classification technique employs a registration procedure that is robust to anatomical variability, including the ventricular enlargement typically associated with neurological diseases and aging. The technique is shown to be comparable in accuracy to manual labeling, and of sufficient sensitivity to robustly detect changes in the volume of noncortical structures that presage the onset of probable Alzheimer's disease."
}
@article{dkt,
  title = "An automated labeling system for subdividing the human cerebral cortex on MRI scans into gyral based regions of interest",
  journal = "NeuroImage",
  volume = "31",
  number = "3",
  pages = "968 - 980",
  year = "2006",
  issn = "1053-8119",
  doi = "https://doi.org/10.1016/j.neuroimage.2006.01.021",
  url = "http://www.sciencedirect.com/science/article/pii/S1053811906000437",
  author = "Rahul S. Desikan and Florent Ségonne and Bruce Fischl and Brian T. Quinn and Bradford C. Dickerson and Deborah Blacker and Randy L. Buckner and Anders M. Dale and R. Paul Maguire and Bradley T. Hyman and Marilyn S. Albert and Ronald J. Killiany",
  abstract = "In this study, we have assessed the validity and reliability of an automated labeling system that we have developed for subdividing the human cerebral cortex on magnetic resonance images into gyral based regions of interest (ROIs). Using a dataset of 40 MRI scans we manually identified 34 cortical ROIs in each of the individual hemispheres. This information was then encoded in the form of an atlas that was utilized to automatically label ROIs. To examine the validity, as well as the intra- and inter-rater reliability of the automated system, we used both intraclass correlation coefficients (ICC), and a new method known as mean distance maps, to assess the degree of mismatch between the manual and the automated sets of ROIs. When compared with the manual ROIs, the automated ROIs were highly accurate, with an average ICC of 0.835 across all of the ROIs, and a mean distance error of less than 1 mm. Intra- and inter-rater comparisons yielded little to no difference between the sets of ROIs. These findings suggest that the automated method we have developed for subdividing the human cerebral cortex into standard gyral-based neuroanatomical regions is both anatomically valid and reliable. This method may be useful for both morphometric and functional studies of the cerebral cortex as well as for clinical investigations aimed at tracking the evolution of disease-induced changes over time, including clinical trials in which MRI-based measures are used to examine response to treatment."
}
 @article{fischl:99,
      AUTHOR = "Fischl, Bruce and Sereno, Martin I. and Dale, Anders",
      TITLE = "Cortical Surface-Based Analysis: II: Inflation, Flattening, and a Surface-Based Coordinate System",
      YEAR = "1999",
      JOURNAL = "NeuroImage",
      VOLUME = "9",
      NUMBER = "2",
      PAGES = "195 - 207",
      ANNOTE = "DOI: 10.1006/nimg.1998.0396"
}
@Article{neuroconductor,
        Author={Muschelli, J. and Gherman, A. and Fortin, J. P. and Avants, B. and Whitcher, B. and Clayden, J. D. and Caffo, B. S. and Crainiceanu, C. M. },
        Title={{N}euroconductor: an {R} platform for medical imaging analysis},
        Journal={Biostatistics},
        Year={2018},
        Month={Jan}
        }
@article{WALHOVD201847,
title = "Healthy minds 0-100 years: Optimising the use of European brain imaging cohorts ('Lifebrain')",
journal = "European Psychiatry",
volume = "50",
pages = "47 - 56",
year = "2018",
note = "Workshop on Schizophrenia and other mental disorders - S. Frangou (Editor in Chief), A. Del Guerra, S. Galderisi (Guest Editors)",
issn = "0924-9338",
doi = "https://doi.org/10.1016/j.eurpsy.2017.12.006",
url = "http://www.sciencedirect.com/science/article/pii/S0924933817330237",
author = "Kristine B. Walhovd and Anders M. Fjell and René Westerhausen and Lars Nyberg and Klaus P. Ebmeier and Ulman Lindenberger and David Bartrés-Faz and William F.C. Baaré and Hartwig R. Siebner and Richard Henson and Christian A. Drevon and Gun Peggy Strømstad Knudsen and Isabelle Budin Ljøsne and Brenda W.J.H. Penninx and Paolo Ghisletta and Ole Rogeberg and Lorraine Tyler and Lars Bertram",
keywords = "Psychiatric disorder, Dementia, Economics and psychiatry, Epidemiology, MRI, Neurodevelopment",
abstract = "The main objective of 'Lifebrain' is to identify the determinants of brain, cognitive and mental (BCM) health at different stages of life. By integrating, harmonising and enriching major European neuroimaging studies across the life span, we will merge fine-grained BCM health measures of more than 5000 individuals. Longitudinal brain imaging, genetic and health data are available for a major part, as well as cognitive and mental health measures for the broader cohorts, exceeding 27,000 examinations in total. By linking these data to other databases and biobanks, including birth registries, national and regional archives, and by enriching them with a new online data collection and novel measures, we will address the risk factors and protective factors of BCM health. We will identify pathways through which risk and protective factors work and their moderators. Exploiting existing European infrastructures and initiatives, we hope to make major conceptual, methodological and analytical contributions towards large integrative cohorts and their efficient exploitation. We will thus provide novel information on BCM health maintenance, as well as the onset and course of BCM disorders. This will lay a foundation for earlier diagnosis of brain disorders, aberrant development and decline of BCM health, and translate into future preventive and therapeutic strategies. Aiming to improve clinical practice and public health we will work with stakeholders and health authorities, and thus provide the evidence base for prevention and intervention."
}
@Manual{R,
    title = {R: A Language and Environment for Statistical Computing},
    author = {{R Core Team}},
    organization = {R Foundation for Statistical Computing},
    address = {Vienna, Austria},
    year = {2019},
    url = {https://www.R-project.org/},
  }
@Manual{python,
    title = {Python: A dynamic, open source programming language},
    author = {{Python Core Team }},
    organization = {Python Software Foundation},
    year = {2015},
    url = {https://www.python.org/},
  }
@manual{MATLAB,
  author = {{MATLAB Core Team }},
  address = {Natick, Massachusetts},
  organization = {The Mathworks, Inc.},
  title = { MATLAB version 8.5.0.197613 (R2015a)},
  year = {2015}
}
@Manual{ggneuro,
  title = {ggneuro: Plotting Functions for Neuroimaging Data in 'ggplot2'},
  author = {John Muschelli},
  year = {2017},
  note = {R package version 0.5.0},
}
@Manual{ggBrain,
    title = {ggBrain: ggplot Brain Images},
    author = {Aaron Fisher},
    year = {2019},
    note = {R package version 0.1}
  }
@Manual{plotly,
    title = {plotly for R},
    author = {Carson Sievert},
    year = {2018},
    url = {https://plotly-r.com},
  }
@Book{ggplot,
    author = {Hadley Wickham},
    title = {ggplot2: Elegant Graphics for Data Analysis},
    publisher = {Springer-Verlag New York},
    year = {2016},
    isbn = {978-3-319-24277-4},
    url = {https://ggplot2.tidyverse.org},
  }
@misc{brainder,
  title = {{Brainder}},
  author = {A. M. Winkler},
  year = {2011},
  howpublished = {\url{https://brainder.org/tag/ply/}},
  note = {Accessed: 2018-10-15}
}


@misc{plotly-ax,
  title = {{plotly} axes},
  author = {Joseph Damiba},
  year = {2019},
  howpublished = {\url{https://plot.ly/r/axes/#modifying-axes-for-3D-plots}},
  note = {Accessed: 2019-04-01}
}
@misc{plotly-tri,
  title = {{plotly} tri-surf},
  author = {Joseph Damiba},
  year = {2019},
  howpublished = {\url{https://plot.ly/r/trisurf/}},
  note = {Accessed: 2019-04-01}
}
@misc{plotly-trisurf,
  title = {{plotly} trisurf2},
  author = {Riddihiman},
  year = {2016},
  howpublished = {\url{https://moderndata.plot.ly/trisurf-plots-in-r-using-plotly/}},
  note = {Accessed: 2019-04-01}
}
@misc{ggseg,
  title = {{ggseg} package website},
  author = {A.M. Mowinckel and D. Vidal-Piñeiro},
  year = {2019},
  howpublished = {\url{https://lcbc-uio.github.io/ggseg/}},
  note = {Accessed: 2019-11-26}
}

@misc{ggseg3d,
  title = {{ggseg3d} package website},
  author = {A.M. Mowinckel and D. Vidal-Piñeiro},
  year = {2019},
  howpublished = {\url{https://lcbc-uio.github.io/ggseg3d/}},
  note = {Accessed: 2019-11-26}
}
@misc{ggsegAnim,
  title = {Get the brain animated! - {Dr.Mowinckels} Blog},
  author = {A.M. Mowinckel},
  year = {2018},
  howpublished = {\url{https://drmowinckels.io/blog/get-the-brain-animated/}},
  note = {Accessed: 2019-04-01}
}
@misc{ggsegIntro,
  title = {Introducing the ggseg R-package for brain segmentations - {Dr.Mowinckels} Blog},
  author = {A.M. Mowinckel},
  year = {2018},
  howpublished = {\url{https://drmowinckels.io/blog/introducing-the-ggseg-r-package-for-brain-segmentations/}},
  note = {Accessed: 2019-04-01}
}
@misc{fsleyes,
  author = {Paul McCarthy},
  title = {FSLeyes},
  month = apr,
  year = 2019,
  doi = {10.5281/zenodo.2630502},
  url = {https://doi.org/10.5281/zenodo.2630502}
}
@Manual{shiny,
    title = {shiny: Web Application Framework for R},
    author = {Winston Chang and Joe Cheng and JJ Allaire and Yihui Xie and Jonathan McPherson},
    year = {2019},
    note = {R package version 1.3.1},
    url = {https://CRAN.R-project.org/package=shiny}
  }
@InProceedings{ binder,
  author    = { {P}roject {J}upyter and {M}atthias {B}ussonnier and {J}essica {F}orde and {J}eremy {F}reeman and {B}rian {G}ranger and {T}im {H}ead and {C}hris {H}oldgraf and {K}yle {K}elley and {G}ladys {N}alvarte and {A}ndrew {O}sheroff and {M} {P}acer and {Y}uvi {P}anda and {F}ernando {P}erez and {B}enjamin {R}agan-{K}elley and {C}arol {W}illing },
  title     = { {B}inder 2.0 - {R}eproducible, interactive, sharable environments for science at scale },
  booktitle = { {P}roceedings of the 17th {P}ython in {S}cience {C}onference },
  pages     = { 113 - 120 },
  year      = { 2018 },
  editor    = { {F}atih {A}kici and {D}avid {L}ippa and {D}illon {N}iederhut and {M} {P}acer },
  doi       = { 10.25080/Majora-4af1f417-011 }
}

@article{vidal_2019,
	title = {Cellular correlates of cortical thinning throughout the lifespan},
	url = {http://biorxiv.org/content/early/2019/03/23/585786.abstract},
	doi = {10.1101/585786},
	abstract = {Changes in cortical thickness occur throughout the lifespan, but the neurobiological substrates are poorly understood. Here, we compared the regional patterns of cortical thinning (Magnetic Resonance Images; \&gt;4000 observations) with those of gene expression for several neuronal and non-neuronal cell types (Allen Human Brain Atlas). Inter-regional profiles of cortical thinning (estimated from MRIs) related to expression profiles for marker genes of CA1 pyramidal cells, astrocytes and microglia during development (less thinning, greater gene expression). The same expression – thinning patterns were mirrored in aging, but in the opposite direction. The results were replicated in independent MRI datasets. Further analyses suggested that the cell type – thinning relationship is facilitated by astrocytic metabolic processes in development and neural projection and synaptic changes in aging. Overall, these findings uncover the neurobiological mechanisms underlying cortical thinning across the lifespan and may contribute to our understanding of the molecular pathways involved in neurodevelopmental and neurodegenerative disorders.},
	journal = {bioRxiv},
	author = {Vidal-Piñeiro, D. and Parker, N. and Shin, J. and French, L. and Jackowski, AP. and Mowinckel, AM. and Patel, Y. and Pausova, Z. and Salum, G. and Sørensen, Ø. and Walhovd, KB and Paus, T. and Fjell, AM},
	month = jan,
	year = {2019},
	pages = {585786}
}
@Article{gganatogram,
   title = {gganatogram:  An R package for modular visualisation of anatograms and tissues based on ggplot2},
   author = {Jesper Maag},
   journal = {f1000research},
   year = {2018},
   note = {Version 1: Awaiting peer review},
   url = {https://f1000research.com/articles/7-1576/v1}
 }

@article{amlien_elaboration_2019,
	title = {Elaboration {Benefits} {Source} {Memory} {Encoding} {Through} {Centrality} {Change}},
	volume = {9},
	issn = {2045-2322},
	url = {https://doi.org/10.1038/s41598-019-39999-1},
	doi = {10.1038/s41598-019-39999-1},
	abstract = {Variations in levels of processing affect memory encoding and subsequent retrieval performance, but it is unknown how processing depth affects communication patterns within the network of interconnected brain regions involved in episodic memory encoding. In 113 healthy adults scanned with functional MRI, we used graph theory to calculate centrality indices representing the brain regions’ relative importance in the memory network. We tested how communication patterns in 42 brain regions involved in episodic memory encoding changed as a function of processing depth, and how these changes were related to episodic memory ability. Centrality changes in right middle frontal gyrus, right inferior parietal lobule and left superior frontal gyrus were positively related to semantic elaboration during encoding. In the same regions, centrality during successful episodic memory encoding was related to performance on the episodic memory task, indicating that these centrality changes reflect processes that support memory encoding through deep elaborative processing. Similar analyses were performed for congruent trials, i.e. events that fit into existing knowledge structures, but no relationship between centrality changes and congruity were found. The results demonstrate that while elaboration and congruity have similar beneficial effects on source memory performance, the cortical signatures of these processes are probably not identical.},
	number = {1},
	journal = {Scientific Reports},
	author = {Amlien, Inge K. and Sneve, Markus H. and Vidal-Piñeiro, Didac and Walhovd, Kristine B. and Fjell, Anders M.},
	month = mar,
	year = {2019},
	pages = {3704}
}






@article{yeo2011,
author = {Yeo, Thomas and B. T. and Krienen, Fenna M. and Sepulcre, Jorge and Sabuncu, Mert R. and Lashkari, Danial and Hollinshead, Marisa and Roffman, Joshua L. and Smoller, Jordan W. and Zöllei, Lilla and Polimeni, Jonathan R. and Fischl, Bruce and Liu, Hesheng and Buckner, Randy L.},
title = {The organization of the human cerebral cortex estimated by intrinsic functional connectivity},
journal = {Journal of Neurophysiology},
volume = {106},
number = {3},
pages = {1125-1165},
year = {2011},
doi = {10.1152/jn.00338.2011},
    note ={PMID: 21653723},

URL = { 
        https://doi.org/10.1152/jn.00338.2011
    
},
eprint = { 
        https://doi.org/10.1152/jn.00338.2011
    
}
,
    abstract = { Information processing in the cerebral cortex involves interactions among distributed areas. Anatomical connectivity suggests that certain areas form local hierarchical relations such as within the visual system. Other connectivity patterns, particularly among association areas, suggest the presence of large-scale circuits without clear hierarchical relations. In this study the organization of networks in the human cerebrum was explored using resting-state functional connectivity MRI. Data from 1,000 subjects were registered using surface-based alignment. A clustering approach was employed to identify and replicate networks of functionally coupled regions across the cerebral cortex. The results revealed local networks confined to sensory and motor cortices as well as distributed networks of association regions. Within the sensory and motor cortices, functional connectivity followed topographic representations across adjacent areas. In association cortex, the connectivity patterns often showed abrupt transitions between network boundaries. Focused analyses were performed to better understand properties of network connectivity. A canonical sensory-motor pathway involving primary visual area, putative middle temporal area complex (MT+), lateral intraparietal area, and frontal eye field was analyzed to explore how interactions might arise within and between networks. Results showed that adjacent regions of the MT+ complex demonstrate differential connectivity consistent with a hierarchical pathway that spans networks. The functional connectivity of parietal and prefrontal association cortices was next explored. Distinct connectivity profiles of neighboring regions suggest they participate in distributed networks that, while showing evidence for interactions, are embedded within largely parallel, interdigitated circuits. We conclude by discussing the organization of these large-scale cerebral networks in relation to monkey anatomy and their potential evolutionary expansion in humans to support cognition. }
}

@article{desterieux,
title = "Automatic parcellation of human cortical gyri and sulci using standard anatomical nomenclature",
journal = "NeuroImage",
volume = "53",
number = "1",
pages = "1 - 15",
year = "2010",
issn = "1053-8119",
doi = "https://doi.org/10.1016/j.neuroimage.2010.06.010",
url = "http://www.sciencedirect.com/science/article/pii/S1053811910008542",
author = "Christophe Destrieux and Bruce Fischl and Anders Dale and Eric Halgren",
keywords = "Anatomy, Atlas, Brain, Cerebral cortex, MRI",
abstract = "Precise localization of sulco-gyral structures of the human cerebral cortex is important for the interpretation of morpho-functional data, but requires anatomical expertise and is time consuming because of the brain's geometric complexity. Software developed to automatically identify sulco-gyral structures has improved substantially as a result of techniques providing topologically correct reconstructions permitting inflated views of the human brain. Here we describe a complete parcellation of the cortical surface using standard internationally accepted nomenclature and criteria. This parcellation is available in the FreeSurfer package. First, a computer-assisted hand parcellation classified each vertex as sulcal or gyral, and these were then subparcellated into 74 labels per hemisphere. Twelve datasets were used to develop rules and algorithms (reported here) that produced labels consistent with anatomical rules as well as automated computational parcellation. The final parcellation was used to build an atlas for automatically labeling the whole cerebral cortex. This atlas was used to label an additional 12 datasets, which were found to have good concordance with manual labels. This paper presents a precisely defined method for automatically labeling the cortical surface in standard terminology."
}

@article {chen,
	author = {Chen, Chi-Hua and Fiecas, Mark and Guti{\'e}rrez, E. D. and Panizzon, Matthew S. and Eyler, Lisa T. and Vuoksimaa, Eero and Thompson, Wesley K. and Fennema-Notestine, Christine and Hagler, Donald J. and Jernigan, Terry L. and Neale, Michael C. and Franz, Carol E. and Lyons, Michael J. and Fischl, Bruce and Tsuang, Ming T. and Dale, Anders M. and Kremen, William S.},
	title = {Genetic topography of brain morphology},
	volume = {110},
	number = {42},
	pages = {17089--17094},
	year = {2013},
	doi = {10.1073/pnas.1308091110},
	publisher = {National Academy of Sciences},
	abstract = {How diverse functional cortical regions develop is an important neuroscience question. Animal experiments show that regional differentiation is controlled by genes that express in a graded and regionalized pattern; however, such investigation in humans is scarce. Using noninvasive imaging techniques to acquire brain structure data of genetically related subjects (i.e., twins), we estimated the spatial pattern of genetic influences on cortical structure. We developed a genetic parcellation of cortical thickness to delineate the boundaries of cortical divisions that are{\textemdash}within each division{\textemdash}maximally under control of shared genetic influences. We also found differences in genetic influences on cortical surface area and thickness along two orthogonal axes. The concept of gradations is crucial for understanding the organization of the human brain.Animal data show that cortical development is initially patterned by genetic gradients largely along three orthogonal axes. We previously reported differences in genetic influences on cortical surface area along an anterior-posterior axis using neuroimaging data of adult human twins. Here, we demonstrate differences in genetic influences on cortical thickness along a dorsal-ventral axis in the same cohort. The phenomenon of orthogonal gradations in cortical organization evident in different structural and functional properties may originate from genetic gradients. Another emerging theme of cortical patterning is that patterns of genetic influences recapitulate the spatial topography of the cortex within hemispheres. The genetic patterning of both cortical thickness and surface area corresponds to cortical functional specializations. Intriguingly, in contrast to broad similarities in genetic patterning, two sets of analyses distinguish cortical thickness and surface area genetically. First, genetic contributions to cortical thickness and surface area are largely distinct; there is very little genetic correlation (i.e., shared genetic influences) between them. Second, organizing principles among genetically defined regions differ between thickness and surface area. Examining the structure of the genetic similarity matrix among clusters revealed that, whereas surface area clusters showed great genetic proximity with clusters from the same lobe, thickness clusters appear to have close genetic relatedness with clusters that have similar maturational timing. The discrepancies are in line with evidence that the two traits follow different mechanisms in neurodevelopment. Our findings highlight the complexity of genetic influences on cortical morphology and provide a glimpse into emerging principles of genetic organization of the cortex.},
	issn = {0027-8424},
	URL = {https://www.pnas.org/content/110/42/17089},
	eprint = {https://www.pnas.org/content/110/42/17089.full.pdf},
	journal = {Proceedings of the National Academy of Sciences}
}


@article{glasser,
	Author = {Glasser, Matthew F. and Coalson, Timothy S. and Robinson, Emma C. and Hacker, Carl D. and Harwell, John and Yacoub, Essa and Ugurbil, Kamil and Andersson, Jesper and Beckmann, Christian F. and Jenkinson, Mark and Smith, Stephen M. and Van Essen, David C.},
	Date = {2016/07/20/online},
	Date-Added = {2019-06-27 13:15:01 +0000},
	Date-Modified = {2019-06-27 13:15:01 +0000},
	Day = {20},
	Journal = {Nature},
	L3 = {10.1038/nature18933; https://www.nature.com/articles/nature18933#supplementary-information},
	M3 = {Article},
	Month = {07},
	Pages = {171 EP  -},
	Publisher = {Macmillan Publishers Limited, part of Springer Nature. All rights reserved. SN  -},
	Title = {A multi-modal parcellation of human cerebral cortex},
	Ty = {JOUR},
	Url = {https://doi.org/10.1038/nature18933},
	Volume = {536},
	Year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1038/nature18933}}

@article{ho,
title = "Decreased volume of left and total anterior insular lobule in schizophrenia",
journal = "Schizophrenia Research",
volume = "83",
number = "2",
pages = "155 - 171",
year = "2006",
issn = "0920-9964",
doi = "https://doi.org/10.1016/j.schres.2005.11.020",
url = "http://www.sciencedirect.com/science/article/pii/S0920996405004998",
author = "Nikos Makris and Jill M. Goldstein and David Kennedy and Steven M. Hodge and Verne S. Caviness and Stephen V. Faraone and Ming T. Tsuang and Larry J. Seidman",
keywords = "Schizophrenia, MRI, Insula",
abstract = "The insula is anatomically situated to be critically involved in many bio-behavioral functions impaired in schizophrenia. Furthermore, its total volume has been shown to be reduced in schizophrenia. In the present study, we tested the hypothesis that in schizophrenia it is the anterior insular lobule (aINSlbl) rather than the posterior insular lobule (pINSlbl) that is smaller, given that limbic system abnormalities are central in schizophrenia and that the affiliations of the limbic system are principally with the anterior insular lobule. We used T1-weighted high resolution magnetic resonance imaging (MRI) to measure the cortical volume of the left and right anterior and posterior insular subdivisions. The subjects included a sample of healthy community controls (N=40) and chronic patients with DSM-III-R schizophrenia (N=41). We correlated insula volumes with positive and negative symptoms. We found that the total aINSlbl, and the left aINSlbl in particular, were significantly volumetrically smaller in schizophrenia compared to controls, and significantly correlated with bizarre behavior. Given that the anterior insular lobule offers anatomic features that allow for MRI-based morphometric analysis, namely its central and circular sulci, this brain structure provides a useful model to test hypotheses regarding genotype–phenotype relationships in schizophrenia using the anterior insular lobule as a candidate endophenotype."
}

@Book{icbm,
    author = {Susumu Mori and S. Wakana and Peter C M van Zijl and L.M. Nagae-Poetscher},
    title = {MRI Atlas of Human White Matter},
    publisher = {Elsevier Science},
    year = {2005},
    isbn = {9780080456164},
    url = {https://www.elsevier.com/books/mri-atlas-of-human-white-matter/mori/978-0-444-51741-8},
  }

@article{jhu,
title = "Tract probability maps in stereotaxic spaces: Analyses of white matter anatomy and tract-specific quantification",
journal = "NeuroImage",
volume = "39",
number = "1",
pages = "336 - 347",
year = "2008",
issn = "1053-8119",
doi = "https://doi.org/10.1016/j.neuroimage.2007.07.053",
url = "http://www.sciencedirect.com/science/article/pii/S105381190700688X",
author = "Kegang Hua and Jiangyang Zhang and Setsu Wakana and Hangyi Jiang and Xin Li and Daniel S. Reich and Peter A. Calabresi and James J. Pekar and Peter C.M. van Zijl and Susumu Mori",
abstract = "Diffusion tensor imaging (DTI) is an exciting new MRI modality that can reveal detailed anatomy of the white matter. DTI also allows us to approximate the 3D trajectories of major white matter bundles. By combining the identified tract coordinates with various types of MR parameter maps, such as T2 and diffusion properties, we can perform tract-specific analysis of these parameters. Unfortunately, 3D tract reconstruction is marred by noise, partial volume effects, and complicated axonal structures. Furthermore, changes in diffusion anisotropy under pathological conditions could alter the results of 3D tract reconstruction. In this study, we created a white matter parcellation atlas based on probabilistic maps of 11 major white matter tracts derived from the DTI data from 28 normal subjects. Using these probabilistic maps, automated tract-specific quantification of fractional anisotropy and mean diffusivity were performed. Excellent correlation was found between the automated and the individual tractography-based results. This tool allows efficient initial screening of the status of multiple white matter tracts."
}

@article{schaefer,
    author = {Schaefer, Alexander and Kong, Ru and Gordon, Evan M and Laumann, Timothy O and Zuo, Xi-Nian and Holmes, Avram J and Eickhoff, Simon B and Yeo, B T Thomas},
    title = "{Local-Global Parcellation of the Human Cerebral Cortex from Intrinsic Functional Connectivity MRI}",
    journal = {Cerebral Cortex},
    volume = {28},
    number = {9},
    pages = {3095-3114},
    year = {2017},
    month = {07},
    abstract = "{A central goal in systems neuroscience is the parcellation of the cerebral cortex into discrete neurobiological “atoms”. Resting-state functional magnetic resonance imaging (rs-fMRI) offers the possibility of in vivo human cortical parcellation. Almost all previous parcellations relied on 1 of 2 approaches. The local gradient approach detects abrupt transitions in functional connectivity patterns. These transitions potentially reflect cortical areal boundaries defined by histology or visuotopic fMRI. By contrast, the global similarity approach clusters similar functional connectivity patterns regardless of spatial proximity, resulting in parcels with homogeneous (similar) rs-fMRI signals. Here, we propose a gradient-weighted Markov Random Field (gwMRF) model integrating local gradient and global similarity approaches. Using task-fMRI and rs-fMRI across diverse acquisition protocols, we found gwMRF parcellations to be more homogeneous than 4 previously published parcellations. Furthermore, gwMRF parcellations agreed with the boundaries of certain cortical areas defined using histology and visuotopic fMRI. Some parcels captured subareal (somatotopic and visuotopic) features that likely reflect distinct computational units within known cortical areas. These results suggest that gwMRF parcellations reveal neurobiologically meaningful features of brain organization and are potentially useful for future applications requiring dimensionality reduction of voxel-wise fMRI data. Multiresolution parcellations generated from 1489 participants are publicly available (https://github.com/ThomasYeoLab/CBIG/tree/master/stable\_projects/brain\_parcellation/Schaefer2018\_LocalGlobal).}",
    issn = {1047-3211},
    doi = {10.1093/cercor/bhx179},
    url = {https://doi.org/10.1093/cercor/bhx179},
    eprint = {http://oup.prod.sis.lan/cercor/article-pdf/28/9/3095/25696343/bhx179.pdf},
}

@ARTICLE{tracula,
  
AUTHOR={Yendiki, Anastasia and Panneck, Patricia and Srinivasan, Priti and Stevens, Allison and Zöllei, Lilla and Augustinack, Jean and Wang, Ruopeng and Salat, David and Ehrlich, Stefan and Behrens, Tim and Jbabdi, Saad and Gollub, Randy and Fischl, Bruce},   
	 
TITLE={Automated Probabilistic Reconstruction of White-Matter Pathways in Health and Disease Using an Atlas of the Underlying Anatomy},      
	
JOURNAL={Frontiers in Neuroinformatics},      
	
VOLUME={5},      

PAGES={23},     
	
YEAR={2011},      
	  
URL={https://www.frontiersin.org/article/10.3389/fninf.2011.00023},       
	
DOI={10.3389/fninf.2011.00023},      
	
ISSN={1662-5196},   
   
ABSTRACT={We have developed a method for automated probabilistic reconstruction of a set of major white-matter pathways from diffusion-weighted MR images. Our method is called TRACULA (TRActs Constrained by UnderLying Anatomy) and utilizes prior information on the anatomy of the pathways from a set of training subjects. By incorporating this prior knowledge in the reconstruction procedure, our method obviates the need for manual interaction with the tract solutions at a later stage and thus facilitates the application of tractography to large studies. In this paper we illustrate the application of the method on data from a schizophrenia study and investigate whether the inclusion of both patients and healthy subjects in the training set affects our ability to reconstruct the pathways reliably. We show that, since our method does not constrain the exact spatial location or shape of the pathways but only their trajectory relative to the surrounding anatomical structures, a set a of healthy training subjects can be used to reconstruct the pathways accurately in patients as well as in controls.}
}

@Manual{magick,
    title = {magick: Advanced Graphics and Image-Processing in R},
    author = {Jeroen Ooms},
    year = {2019},
    note = {R package version 2.2},
    url = {https://CRAN.R-project.org/package=magick},
  }
  
@article{cran,
author = {Hornik, Kurt},
title = {The Comprehensive R Archive Network},
journal = {WIREs Computational Statistics },

volume = {4},
number = {4},
pages = {394-398},
keywords = {R, R sources and binaries, R package repositories, collaborative software development, software quality, statistical computing, knowledge domain},
doi = {10.1002/wics.1212},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/wics.1212},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/wics.1212},
abstract = {Abstract The Comprehensive R Archive Network (CRAN) is a network of sites acting as the primary web service distributing R sources and binaries, extension packages, and documentation. We discuss this functionality in more detail, with particular emphasis on the CRAN package repository, and its underlying design and operation principles. WIREs Comput Stat 2012 doi: 10.1002/wics.1212 This article is categorized under: Applications of Computational Statistics > Organizations and Publications},
year = {2012}
}

@article{fsl,
  doi = {10.1016/j.neuroimage.2008.10.055},
  url = {https://doi.org/10.1016/j.neuroimage.2008.10.055},
  year = {2009},
  month = mar,
  publisher = {Elsevier {BV}},
  volume = {45},
  number = {1},
  pages = {S173--S186},
  author = {Mark W. Woolrich and Saad Jbabdi and Brian Patenaude and Michael Chappell and Salima Makni and Timothy Behrens and Christian Beckmann and Mark Jenkinson and Stephen M. Smith},
  title = {Bayesian analysis of neuroimaging data in {FSL}},
  journal = {{NeuroImage}}
}

@misc{ggsegExt12_lcbc,
  author = {A.M. Mowinckel and D. Vidal-Piñeiro},
  title = {ggsegExtra/extras - LCBC surface files},
  howpublished = {\url{https://github.com/LCBC-UiO/ggsegExtra/tree/master/extras}},
  month = {},
  year = {},
  note = {(Accessed on 11/28/2019)}
}

